A space-time finite element method for the eddy current approximation of rotating electric machines

In this paper we formulate and analyze a space-time finite element method for the numerical simulation of rotating electric machines where the finite element mesh is fixed in space-time domain. Based on the Babu\v{s}ka--Ne\v{c}as theory we prove unique solvability both for the continuous variational formulation and for a standard Galerkin finite element discretization in the space-time domain. This approach allows for an adaptive resolution of the solution both in space and time, but it requires the solution of the overall system of algebraic equations. While the use of parallel solution algorithms seems to be mandatory, this also allows for a parallelization simultaneously in space and time. This approach is used for the eddy current approximation of the Maxwell equations which results in an elliptic-parabolic interface problem. Numerical results for linear and nonlinear constitutive material relations confirm the applicability, efficiency and accuracy of the proposed approach.

==> tmp_paper_abstract.tex <==
\begin{abstract}
  In this paper we formulate and analyze a space-time finite element
  method for the numerical simulation of rotating electric machines where
  the finite element mesh is fixed in space-time domain.
  Based on the Babu\v{s}ka--Ne\v{c}as theory we prove unique solvability
  both for the continuous variational formulation and for a standard Galerkin
  finite element discretization in the space-time domain. This approach
  allows for an adaptive resolution of the solution both in space and time,
  but it requires the solution of the overall system of algebraic equations.
  While the use of parallel solution algorithms seems to be mandatory,
  this also allows for a parallelization simultaneously in space and time.
  This approach is used for the eddy current approximation of the Maxwell
  equations which results in an elliptic-parabolic interface problem.
  Numerical results for linear and nonlinear constitutive material relations
  confirm the applicability, efficiency and accuracy of the proposed
  approach.
\end{abstract}

\begin{keywords}
  Maxwell equations, eddy current approximation, space-time finite element
  methods
\end{keywords}

\begin{MSCcodes}
35K05, 35Q60, 65M60, 65Z05
\end{MSCcodes}


==> tmp_paper_header.tex <==
  \title{A space-time finite element method for the eddy current
    approximation of rotating electric machines\footnote{P\lowercase{reliminary numerical results of this space-time finite element method are
accepted for publication in the proceedings of the 27th} I\lowercase{nternational }C\lowercase{onference
on }D\lowercase{omain }D\lowercase{ecomposition }M\lowercase{ethods in }S\lowercase{cience and }E\lowercase{ngineering, see \cite{GaGoSt23}}.}}
\author{Peter Gangl\thanks{Johann Radon Institute for Computational and
    Applied Mathematics, Altenberger Strasse 69, 4040 Linz, Austria
    (\email{peter.gangl@ricam.oeaw.ac.at}).}
  \and Mario Gobrial\thanks{Institut f\"{u}r Angewandte Mathematik, \,
    Technische Universit\"{a}t Graz, \, Steyrergasse 30, \, 8010 Graz, Austria
    (\email{gobrial@math.tugraz.at}, \email{o.steinbach@tugraz.at}).}
\and Olaf Steinbach\footnotemark[3]}

% Custom SIAM macro to insert headers
\headers{Space-time FEM for the approximation
  of rotating electric machines}
{Peter Gangl, Mario Gobrial, and Olaf Steinbach}

